Expectation Propagation in Gaussian Process Dynamical Systems: Extended Version

Rich and complex time-series data, such as those generated from engineering systems, financial markets, videos or neural recordings, are now a common feature of modern data analysis. Explaining the phenomena underlying these diverse data sets requires flexible and accurate models. In this paper, we promote Gaussian process dynamical systems (GPDS) as a rich model class that is appropriate for such analysis. In particular, we present a message passing algorithm for approximate inference in GPDSs based on expectation propagation. By posing inference as a general message passing problem, we iterate forward-backward smoothing. Thus, we obtain more accurate posterior distributions over latent structures, resulting in improved predictive performance compared to state-of-the-art GPDS smoothers, which are special cases of our general message passing algorithm. Hence, we provide a unifying approach within which to contextualize message passing in GPDSs.

==> sec_background.tex <==
\subsection{Expectation Propagation}
%
Expectation propagation (EP)~\cite{Minka2001a} is an accurate
deterministic inference algorithm, based on generalizations of Assumed
Density Filtering~\cite{Boyen1998}. EP is derived using a factor-graph
representation of a model, which represents the joint distribution
over the latent variables $p(\vec x)$ as a product of model factors
$f_i(\vec x)$.  EP then specifies a message passing algorithm in which
$p(\vec x)$ is approximated by a distribution $q (\vec x)$, which is a
product of approximate messages $q_i(\vec x)$, and is the best
tractable approximation, such that the he KL-divergence KL$(p||q)$ is
minimized.

This is realised practically in two steps: a \textit{projection} step in which each approximate message $q_i(\vec x)$ is computed in the context of neighbouring factors, and an \textit{updating} step in which the marginal distribution $\vec q(x_i)$ is updated using the new message. For every factor in the graph, the required computation is:
\begin{align}
q_{i}(\vec x_j) &= \frac{\proj{f_{i}(\vec
    x_j)q^{\setminus i}(\vec x_j)}}{q^{\setminus i} (\vec x_j)}\,,
\label{eq:update measurement message}
\end{align}
where the operator $\texttt{proj}[\vec x]$ is a moment-matching operator that projects its argument to the closest Gaussian distribution and returns its moments -- these moments are obtained using the normalizing constant of the \texttt{proj}-argument and computing is derivatives which yield the required moments. 


\begin{algorithm}[t]
  \caption{EP for time series models}
\begin{algorithmic}[1]
\State Initialize all factors\slash sites $q_i$ to $\gauss{\vec
  0}{\infty\mat I}$
\State Initialize $q(\vec x_1)$ to the prior $p(x_1)$ and all other
marginals $\vec x_{t\neq 1}=\gauss{\vec 0}{10^{10}\mat I}$ 
\Repeat
\For{$t = 1$ to $T$}
\For {all factors $q_i(\vec x_t)$, where $i=\fwd,\up,\back$}
\State Compute cavity distribution $q\noti(\vec x_t)=q(\vec
x_t)/q_i(\vec x_t)$
\State Compute moments of $f_i(\vec x_t)q\noti(\vec x_t)$, e.g., via the
log-partition function
\State Update the posterior $q(\vec x_t)$ and the approximate factor
$q_i(\vec x_t)$ 
\EndFor
\EndFor
\Until Convergence or maximum number of iterations exceeded
\end{algorithmic}
\end{algorithm}

We describe the steps of EP in detail here following \citep{Minka2001,
  Minka2008}. Assume that we have a collection of random variables
$\vec x_1,\dotsc, \vec x_n$. The EP updates are computed as follows:
\begin{enumerate}
\item Initialize all site distributions $q_i$ (factors) to 1 if no
  more specific prior is available: In a dynamic system, for example,
  the first forward message is initialized by the prior over the
  latent variable.
\item For all latent variables $\vec x_j$ and all sites $f_i(\vec
  x_j)$ do
\begin{enumerate}
\item Remove site $q_i(\vec x_j)$ from the posterior $q(\vec
  x_j)=\gauss{\vec \mu}{\mat\Sigma}$ and compute the ``cavity
  distribution'' $q(\vec x_j)\noti$ by Gaussian division (assuming
  that the approximate sites $q_i$ are all Gaussian). We obtain then
  $q\noti(\vec x_j) = \gaussx{\vec x_j}{\vec
    \mu\noti}{\mat\Sigma\noti}$ with
%
\begin{align}
  \mat\Sigma\noti = (\mat\Sigma\inv -
  \mat\Sigma_i\inv)\inv\,,\qquad\vec \mu\noti =
  \mat\Sigma\noti(\mat\Sigma\inv\vec \mu - \mat\Sigma_i\inv\vec \mu_i)
\end{align}
% 
\item Compute the normalization constant using the true factor
  $f_i(\vec x_j)$
%
\begin{align}
Z_i\inv(\vec\mu\noti,\mat\Sigma\noti) &= \int f_i(\vec x_j) q\noti(\vec
x_j) \d\vec x_j
\end{align}
\item By using properties of exponential family distributions, we
  update the mean $\vec\mu_j$ and covariance $\mat\Sigma_j$ of the
  Gaussian marginal $q(\vec x_j)=\gaussx{\vec
    x_j}{\vec\mu_j}{\mat\Sigma_j}$ according to
\begin{align}
  \vec\mu_j &= \vec\mu\noti + \mat\Sigma\noti\nabla_m\T\,, \qquad
  \mat\Sigma_j = \mat\Sigma\noti - \mat\Sigma\noti(\nabla_m\T\nabla_m
  - 2\nabla_s)\mat\Sigma\noti \label{eq:factored distribution update}
\end{align}
%
where we defined the short-hand notations
%
\begin{align}
  \vec \nabla_m \coloneqq \nabla_{\vec\mu\noti}\log Z_i\inv\,, \qquad
  \mat \nabla_s \coloneqq \nabla_{\mat\Sigma\noti}\log Z_i\inv
\end{align}
%
for the derivatives of the log-normalization constant with respect to
the mean and the covariance of the cavity distribution, respectively.
Note that $\nabla_m$ is a row vector. 
\item Update the mean $\vec\mu_i$, the covariance $\mat\Sigma_i$, and
  the normalization constant $s_i$ of the site $\tilde f_i$ either by
  Gaussian division of $q(\vec x_j)/q\noti(\vec x_j)$ or according to
\begin{align}
\mat\Sigma_i &= (\nabla_m\T\nabla_m - 2\nabla_s)\inv -
\mat\Sigma\noti\label{eq:site cov update}\\
\vec\mu_i &= \vec\mu\noti + (\nabla_m\T\nabla_m -
2\nabla_s)\inv\nabla_m\T\label{eq:site mean update}\\
s_i &=  Z_i\inv\sqrt{|\mat I + \mat\Sigma\noti\mat\Sigma_i\inv|} \exp\big(
+\tfrac{1}{2}(\nabla_m(\nabla_m\T\nabla_m - 2\nabla_s)\inv\nabla_m\T)
\big)\label{eq:site normalization update}
\end{align}
% 
\end{enumerate}
\end{enumerate}







%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2012"
%%% End: 

